Unfolding Semantics of the Untyped {\lambda}-Calculus with letrec

We investigate the relationship between finite terms in {\lambda}-letrec, the {\lambda}-calculus with letrec, and the infinite {\lambda}-terms they express. We say that a lambda-letrec term expresses a lambda-term if the latter can be obtained as an infinite unfolding of the former. Unfolding is the process of substituting occurrences of function variables by the right-hand side of their definition. We consider the following questions: (i) How can we characterise those infinite {\lambda}-terms that are {\lambda}-letrec-expressible? (ii) Given two {\lambda}-letrec terms, how can we determine whether they have the same unfolding? (iii) Given a {\lambda}-letrec term, can we find a more compact version of the term with the same unfolding? To tackle these questions we introduce and study the following formalisms: (i) a rewriting system for unfolding {\lambda}-letrec terms into {\lambda}-terms (ii) a rewriting system for `observing' {\lambda}-terms by dissecting their term structure (iii) higher-order and first-order graph formalisms together with translations between them as well as translations from and to {\lambda}-letrec. We identify a first-order term graph formalism on which bisimulation preserves and reflects the unfolding semantics of {\lambda}-letrec and which is closed under functional bisimulation. From this we derive efficient methods to determine whether two terms are equivalent under infinite unfolding and to compute the maximally shared form of a given {\lambda}-letrec term.

==> figs/Makefile <==
.SUFFIXES:

SVGFILES=$(wildcard *.svg)

all: pdfs removePageGroups

pdfs: $(SVGFILES:.svg=.pdf)

%.pdf: %.svg
	inkscape -A $@ $<
	sed -i '\/Group <</,+5d' $@

removePageGroups:
	find . -name "*.pdf" -type f -exec sed -i '\/Group <</,+5d' {} \;


==> figs/pstricks/named/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs

pdfs: $(TEXFILES:.tex=-st.pdf) $(TEXFILES:.tex=-sst.pdf) $(TEXFILES:.tex=-ltg-u.pdf) $(TEXFILES:.tex=-ltg-l.pdf)

%-st.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/syntaxtree}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%-sst.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/scopedsyntaxtree}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%-ltg-u.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg}' >> $@
	echo '\\newcommand\\nlabel[1]{}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%-ltg-l.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg}' >> $@
	echo '\\newcommand\\nlabel[1]{#1}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

include mk/figure.mk


==> figs/pstricks/nameless/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs

#pdfs: $(TEXFILES:.tex=-lgr.pdf) $(TEXFILES:.tex=-sgr.pdf) $(TEXFILES:.tex=-ltg-u.pdf) $(TEXFILES:.tex=-ltg-l.pdf) $(TEXFILES:.tex=-ltg-u-bl.pdf) $(TEXFILES:.tex=-ltg-l-bl.pdf)
pdfs: $(TEXFILES:.tex=-lgr.pdf)

%-lgr.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/lambdagraph}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

#%-sgr.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/scopedgraph}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@

#%-ltg-u-bl.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg-bl}' >> $@
#	echo '\\newcommand\\nlabel[1]{}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@
#
#%-ltg-l-bl.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg-bl}' >> $@
#	echo '\\newcommand\\nlabel[1]{#1}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@
#
#%-ltg-u.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg}' >> $@
#	echo '\\newcommand\\nlabel[1]{}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@
#
#%-ltg-l.gtx: %.tex
#	cat mk/prelude.tex > $@
#	echo '\\input{macros/ltg}' >> $@
#	echo '\\newcommand\\nlabel[1]{#1}' >> $@
#	cat $< >> $@
#	cat mk/postlude.tex >> $@

include mk/figure.mk


==> figs/pstricks/prefixed/Makefile <==
# create a picture for each file containing a Lagtx fragment in the directory

# disable implicit rules
.SUFFIXES:

TEXFILES=$(wildcard *.tex)

#noflags:
#	make -r default

default: pdfs

pdfs: $(TEXFILES:.tex=-ltg.pdf) $(TEXFILES:.tex=-lhotg.pdf) $(TEXFILES:.tex=-naive.pdf)

%-ltg.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/ltg}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%-naive.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/naive}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

%-lhotg.gtx: %.tex
	cat mk/prelude.tex > $@
	echo '\\input{macros/lhotg}' >> $@
	cat $< >> $@
	cat mk/postlude.tex >> $@

include mk/figure.mk


==> stmary.tex <==
% Loads stmaryrd symbols for 10pt plain TeX documents.
% Use \stmaryrdninepoint for nine point documents.
% Use \stmaryrdelevenpoint for eleven point documents.
% Use \stmaryrdtwelvepoint for twelve point documents.
%
% See stmaryrd docs for the symbols available and the commands to
% access them.

\edef\restoreallcatcodes{%
   \catcode`\noexpand\@=\number\catcode`\@\relax
   \catcode`\noexpand\!=\number\catcode`\!\relax}

\newfam\stmaryrdfam

\font\stmaryfiv  stmary5
\font\stmarysix  stmary6
\font\stmarysev  stmary7
\font\stmaryegt  stmary8
\font\stmarynin  stmary9
\font\stmaryten  stmary10
\font\stmaryelv  stmary10 at10.95pt
\font\stmarytwl  stmary10 at12pt

\def\stmaryrdninepoint{%
  \textfont\stmaryrdfam\stmarynin
  \scriptfont\stmaryrdfam\stmarysev
  \scriptscriptfont\stmaryrdfam\stmaryfiv}

\def\stmaryrdtenpoint{%
  \textfont\stmaryrdfam\stmaryten
  \scriptfont\stmaryrdfam\stmarysev
  \scriptscriptfont\stmaryrdfam\stmaryfiv}

\def\stmaryrdelevenpoint{%
  \textfont\stmaryrdfam\stmaryelv
  \scriptfont\stmaryrdfam\stmaryegt
  \scriptscriptfont\stmaryrdfam\stmarysix}

\def\stmaryrdtwelvepoint{%
  \textfont\stmaryrdfam\stmarytwl
  \scriptfont\stmaryrdfam\stmaryegt
  \scriptscriptfont\stmaryrdfam\stmarysix}

\catcode`\@=11
\def\hexnumber@#1{\ifcase#1%
  0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or
  8\or 9\or A\or B\or C\or D\or E\or F\fi}

\catcode`\!\active
\edef!{\hexnumber@\stmaryrdfam}

\mathchardef\shortleftarrow"3!00
\mathchardef\shortrightarrow"3!01
\mathchardef\shortuparrow"3!02
\mathchardef\shortdownarrow"3!03
\mathchardef\Yup"2!04
\mathchardef\Ydown"2!05
\mathchardef\Yleft"2!06
\mathchardef\Yright"2!07
\mathchardef\varcurlyvee"2!08
\mathchardef\varcurlywedge"2!09
\mathchardef\minuso"2!0A
\mathchardef\baro"2!0B
\mathchardef\sslash"2!0C
\mathchardef\bbslash"2!0D
\mathchardef\moo"2!0E
\mathchardef\varotimes"2!0F
\mathchardef\varoast"2!10
\mathchardef\varobar"2!11
\mathchardef\varodot"2!12
\mathchardef\varoslash"2!13
\mathchardef\varobslash"2!14
\mathchardef\varocircle"2!15
\mathchardef\varoplus"2!16
\mathchardef\varominus"2!17
\mathchardef\boxast"2!18
\mathchardef\boxbar"2!19
\mathchardef\boxdot"2!1A
\mathchardef\boxslash"2!1B
\mathchardef\boxbslash"2!1C
\mathchardef\boxcircle"2!1D
\mathchardef\boxbox"2!1E
\mathchardef\boxempty"2!1F
\mathchardef\lightning"0!20
\mathchardef\merge"2!21
\mathchardef\vartimes"2!22
\mathchardef\fatsemi"2!23
\mathchardef\sswarrow"3!24
\mathchardef\ssearrow"3!25
\mathchardef\curlywedgeuparrow"3!26
\mathchardef\curlywedgedownarrow"3!27
\mathchardef\fatslash"2!28
\mathchardef\fatbslash"2!29
\mathchardef\lbag"2!2A
\mathchardef\rbag"2!2B
\mathchardef\varbigcirc"2!2C
\mathchardef\leftrightarroweq"3!2D
\mathchardef\curlyveedownarrow"3!2E
\mathchardef\curlyveeuparrow"3!2F
\mathchardef\nnwarrow"3!30
\mathchardef\nnearrow"3!31
\mathchardef\leftslice"2!32
\mathchardef\rightslice"2!33
\mathchardef\varolessthan"2!34
\mathchardef\varogreaterthan"2!35
\mathchardef\varovee"2!36
\mathchardef\varowedge"2!37
\mathchardef\talloblong"2!38
\mathchardef\interleave"2!39
\mathchardef\obar"2!3A
\mathchardef\obslash"2!3B
\mathchardef\olessthan"2!3C
\mathchardef\ogreaterthan"2!3D
\mathchardef\ovee"2!3E
\mathchardef\owedge"2!3F
\mathchardef\oblong"2!40
\mathchardef\inplus"3!41
\mathchardef\niplus"3!42
\mathchardef\nplus"2!43
\mathchardef\subsetplus"3!44
\mathchardef\supsetplus"3!45
\mathchardef\subsetpluseq"3!46
\mathchardef\supsetpluseq"3!47
\mathchardef\Lbag"4!48
\mathchardef\Rbag"5!49

\mathchardef\llparenthesis"4!4C
\mathchardef\rrparenthesis"5!4D
\mathchardef\binampersand"4!4E
\mathchardef\bindnasrepma"5!4F
\mathchardef\trianglelefteqslant"3!50
\mathchardef\trianglerighteqslant"3!51
\mathchardef\ntrianglelefteqslant"3!52
\mathchardef\ntrianglerighteqslant"3!53
\mathchardef\llfloor"4!54
\mathchardef\rrfloor"5!55
\mathchardef\llceil"4!56
\mathchardef\rrceil"5!57
\mathchardef\arrownot"3!58
\mathchardef\Arrownot"3!59
\mathchardef\Mapstochar"3!5A
\mathchardef\mapsfromchar"3!5B
\mathchardef\Mapsfromchar"3!5C
\mathchardef\leftrightarrowtriangle"2!5D
\mathchardef\leftarrowtriangle"3!5E
\mathchardef\rightarrowtriangle"3!5F
\mathchardef\bigtriangledown"1!60
\mathchardef\bigtriangleup"1!61
\mathchardef\bigcurlyvee"1!62
\mathchardef\bigcurlywedge"1!63
\mathchardef\bigsqcap"1!64
\mathchardef\bigbox"1!65
\mathchardef\bigparallel"1!66
\mathchardef\biginterleave"1!67
\mathchardef\bignplus"1!70

\edef\llbracket{\delimiter"4!4A!71}
\edef\rrbracket{\delimiter"5!4B!79}

\def\@tempa#1{
  \def\varcopyright{{\ooalign{\hfil\raise.07ex\hbox{c}\hfil\crcr\mathhexbox#12C}}}}
\expandafter\@tempa!

% The long arrow negations.

\def\longarrownot{\mathrel{\mkern5.5mu\arrownot\mkern-5.5mu}}
\def\Longarrownot{\mathrel{\mkern5.5mu\Arrownot\mkern-5.5mu}}

% The variants on \mapsto:

\def\Mapsto{\Mapstochar\Rightarrow}
\def\mapsfrom{\leftarrow\mapsfromchar}
\def\Mapsfrom{\Leftarrow\Mapsfromchar}
\def\Longmapsto{\Mapstochar\Longrightarrow}
\def\longmapsfrom{\longleftarrow\mapsfromchar}
\def\Longmapsfrom{\Longleftarrow\Mapsfromchar}

\restoreallcatcodes

\stmaryrdtenpoint

